Distortion-Based Outer-Bounds for Channels with Rate-Limited Feedback

We present a new technique to obtain outer-bounds on the capacity region of networks with ultra low-rate feedback. We establish a connection between the achievable rates in the forward channel and the minimum distortion that can be attained over the feedback channel.

==> Achievability_XC.tex <==
X-Channels can be thought of as a generalization of several known problems such as interference channels, broadcast channels, multiple-access channels, and multicast channels. In the previous section, we developed a set of new outer-bounds for this problem. In this section, we show that a careful combination of the capacity-achieving strategies for other known known problems will achieve the capacity region of the X-Channel. However, in Section~\ref{Section:Gen}, we show that if we treat the X-Channel as a number of disjoint sub-problems, we may not achieve the capacity. In fact, in some regimes, we need to interleave the capacity-achieving strategies of different sub-problems and execute them simultaneously.

To describe the transmission strategy, we first present two examples. The first example describes a symmetric scenario associated with Fig.~\ref{Fig:CommonRates}(b), and the second example describes a scenario in which transmitters achieve unequal rates. After the examples, we present the general scheme.

\begin{figure}[ht]
\centering
\subfigure[]{\includegraphics[height = 2in]{FiguresPDF/Sub-Multicast.pdf}}
%
\subfigure[]{\includegraphics[height = 2in]{FiguresPDF/Sub-IC.pdf}}
%
\subfigure[]{\includegraphics[height = 2in]{FiguresPDF/Sub-ICSwapped.pdf}}
\caption{\it (a) The two-user multicast channel and its capacity region, the capacity can be achieved without using the delayed CSI; (b) The two-user binary fading interference channel and its capacity region; (c) The two-user binary fading interference channel with swapped IDs and its capacity region.\label{Fig:ExSymmetric}}
\end{figure}

\subsection{Example~1:~Symmetric Sum-Rate of Fig.~\ref{Fig:CommonRates}(b)}
\label{Section:Sym}

Suppose for $p = 0.5$, we wish to achieve the sum-capacity of $\mathcal{C}_{\sf SUM}\left( 1/4 \right) = 0.85$, as defined in (\ref{Eq:CSUM}), with
\begin{align}
\label{Eq:RatesEx1}
& R_{01} = R_{02} = 1/8, \nonumber \\
& R_{11} = R_{12} = R_{21} = R_{22} = 0.15,
\end{align}
as shown in Fig.~\ref{Fig:CommonRates}(b). 

For this particular example, we treat the X-Channel as three separate problems listed below at different times, and we show that this strategy achieves the capacity.
\begin{itemize}

\item For the first third of the communication block, we treat the X-Channel as a two-user multicast channel as depicted in Fig.~\ref{Fig:ExSymmetric}(a) in which each transmitter has a message for {\it both} receivers. For the two-user multicast channel with fading parameter $1/2$, the capacity region matches that of the multiple-access channel formed at each receiver~\cite{AlirezaBFICDelayed} and depicted in Fig.~\ref{Fig:ExSymmetric}(a) as well.

\item For the second third of the communication block, we treat the X-Channel as a two-user interference channel in which ${\sf Tx}_j$ wishes to communicated with ${\sf Rx}_j$, see Fig.~\ref{Fig:ExSymmetric}(b). The capacity region of this problem is given in~\cite{AlirezaBFICDelayed} and depicted in Fig.~\ref{Fig:ExSymmetric}(b).

\item During the final third of the communication block, we treat the X-Channel as a two-user interference channel with swapped IDs in which ${\sf Tx}_j$ wishes to communicated with ${\sf Rx}_{\bar{j}}$, see Fig.~\ref{Fig:ExSymmetric}(c). In the homogeneous setting of this work, the capacity region of this interference channel with swapped IDs matches that of the previous case and is depicted in Fig.~\ref{Fig:ExSymmetric}(c).

\end{itemize}

\noindent {\bf Achievable Rates}: We note that as the communication block length, $n$, goes to infinity, so do the communication block lengths for each sub-problem. Thus, during the first third of the communication block, we can achieve symmetric common rates arbitrary close to $\left( 3/8, 3/8 \right)$. Normalizing to the total communication block, we achieve $\left( R_{01}, R_{02} \right) = \left( 1/8, 1/8 \right)$ which matches the requirements of (\ref{Eq:RatesEx1}). From~\cite{AlirezaBFICDelayed} we know that for the two-user binary fading interference channel with delayed CSIT and $p =1/2$, we can achieve symmetric rates of $\left( 0.45, 0.45 \right)$. Normalizing to the total communication block, we achieve $\left( R_{11}, R_{22} \right) = \left( 0.15, 0.15 \right)$ which matches the requirements of (\ref{Eq:RatesEx1}). Finally, during  the final third of the communication block we treat the problem as a two-user interference channel with swapped IDs in which we can achieve symmetric rates of $\left( 0.45, 0.45 \right)$. Normalizing to the total communication block, we achieve $\left( R_{21}, R_{12} \right) = \left( 0.15, 0.15 \right)$ which again matches the requirements of (\ref{Eq:RatesEx1}). Thus, with splitting up the X-Channel into a combination of three known sub-problems, we can achieve the outer-bound region described in Theorem~\ref{THM:Out_XC}.

\begin{figure}[ht]
\centering
\subfigure[]{\includegraphics[height = 1.5in]{FiguresPDF/Sub-BCCommon.pdf}}
%
\subfigure[]{\includegraphics[height = 2in]{FiguresPDF/Sub-BCDelayed.pdf}}
\caption{\it (a) The two-user broadcast channel with a single common message; (b) The two-user broadcast channel with delayed CSIT and private messages, and its capacity region.\label{Fig:ExUnequal}}
\end{figure}


\subsection{Example~2:~Unequal Rates}
\label{Section:Unequal}

In the previous subsection we focused on a symmetric setting. Here, we discuss a scenario in which transmitters have different types of messages with different rates for each receiver. More precisely, we consider the region in Fig.~\ref{Fig:CommonRates}(c) for $p = 0.5$, and
\begin{align}
\label{Eq:RatesEx2}
& R_{01} = 1/2, \nonumber \\
& R_{02} = 0, \nonumber \\
& R_{11} = R_{21} = 0, \nonumber \\
& R_{12} = R_{22} = 0.15,
\end{align}

In this case, we can think of the X-Channel in this case as two sub-problems that coexist at the same time as described below.
\begin{itemize}

\item The Binary Fading Broadcast Channel from ${\sf Tx}_1$ as in Fig.~\ref{Fig:ExUnequal}(a) in which a single message is intended for both receivers. For this problem, the capacity can be achieved using a point-to-point erasure code of rate $1/2$.

\item The Binary Fading Broadcast Channel from ${\sf Tx}_2$ as in Fig.~\ref{Fig:ExUnequal}(b) with delayed CSIT in which the transmitter has a private message for each receiver. For this problem, the capacity region is given in~\cite{jolfaei1993new,georgiadis2009broadcast} and depicted Fig.~\ref{Fig:ExUnequal}(b). As described below, in order to be able to decode the messages in the presence of the broadcast channel from ${\sf Tx}_1$, we first encode $W_{12}$ and $W_{22}$ using point-to-point erasure codes of rate $1/2$, and treat the resulting codes as the input messages to the broadcast channel of Fig.~\ref{Fig:ExUnequal}(b).   

\end{itemize}

\noindent {\bf Achievable Rates}: At each receiver the received signal from ${\sf Tx}_2$ is corrupted (erased) half of times by the signal from ${\sf Tx}_1$. As a result, when we implement the capacity-achieving strategy of~\cite{jolfaei1993new,georgiadis2009broadcast}, we only deliver half of the bits intended for each receiver. However, since we first encode $W_{12}$ and $W_{22}$ using point-to-point erasure codes of rate $1/2$, obtaining half of the bits is sufficient for reliable decoding of $W_{12}$ and $W_{22}$. Thus, we achieve
\begin{align}
\left( R_{12}, R_{22} \right) = \frac{1}{2} \left( 0.3, 0.3 \right) = \left( 0.15, 0.15 \right), 
\end{align}
which again matches the requirements of (\ref{Eq:RatesEx2}). At the end of the communication block, receivers decode $W_{12}$ and $W_{22}$, and remove the contribution of ${\sf Tx}_2$ from their received signals. After removing the contribution of $X_2^n$, the problem is identical to the broadcast channel from ${\sf Tx}_1$ as in Fig.~\ref{Fig:ExUnequal}(a) for which we can achieve a common rate $R_{02}$ of $1/2$. 


\subsection{A Note on the X-Channel vs. the Interference Channel}
\label{Section:XCvsIC}


\begin{figure}[ht]
\centering
\includegraphics[height = 3in]{FiguresPDF/SumCapacity.pdf}
\caption{\it The sum-capacity of the X-Channel vs. that of the Interference Channel. To have a fair comparison, in the X-Channel we set $R_0 = 0$.\label{Fig:SumCapacity}}
\end{figure}


An important difference between the X-Channel and the interference channel is the fact that in the latter scenario, the individual rates are limited by the capacity of a point-to-point channel, \emph{i.e.} $p$. As a result, for the interference channel, we have~\cite{AlirezaBFICDelayed}:
\begin{align} 
\text{Interference~Channel:~}\sup{\left( R_1+R_2 \right)} = \min\left\{  2p, \frac{2\beta \left( 1-q^2\right)}{1+\beta} \right\}.
\end{align}
However, in the X-Channel no such limitation exists, and we have
\begin{align} 
\text{X-Channel:~}\sup{\left(R_1+R_2\right)} = \frac{2\beta \left\{ \left( 1-q^2\right) - R_0 \right\}}{1+\beta}.
\end{align}  
The difference is depicted in Fig.~\ref{Fig:SumCapacity} for $R_0 = 0$. This means that if we naively try to use the capacity-achieving strategies of the sub-problems independently, we cannot achieve the capacity region of the X-Channel. The key idea to overcome this challenge is to take an approach similar to the one we presented in Section~\ref{Section:Unequal} and run different strategies simultaneously as described below. 


\subsection{Transmission Strategy: Maximum Symmetric Point}
\label{Section:Gen}

The two examples we have provided so far demonstrate the key ideas behind the transmission strategy. We now present a systematic way of utilizing the capacity-achieving strategies of other problems, such as the interference channel and the multicast channel, in order to achieve the capacity region of the X-Channel. % As mentioned before, our results rely on the achievability strategy of other well-known problems, including the two-user erasure interference channel with delayed CSIT. Since the capacity region of this latter problem is only known for the conditions of Theorem~\ref{THM:Ach_XC}, we could not achieve the outer-bound region of Theorem~\ref{THM:Out_XC} for all values of erasure probabilities.

Fix $0 \leq R_0 \leq (1-q^2)$. Then, our goal is the maximum sum-rate point derived from the outer-bounds of Theorem~\ref{THM:Out_XC}. In other words, we need to achieve
\begin{align}
\label{Eq:SymGeneral}
& 0 \leq R_0 \leq (1-q^2), \nonumber \\
& R_1 = R_2 = \frac{\beta \left[ (1-q^2) - R_0 \right]}{1+\beta}.
\end{align}
For the homogeneous setting that we consider in this work, the maximum sum-rate is attained when all $R_{ij}$'s are equal, $i,j \in \{ 1, 2\}$. We first focus on this maximum sum-rate corner point. % and all other corner points are achieved by tuning the 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%Fix $(R_{01},R_{02},R_{11},R_{12},R_{21},R_{22})$ satisfying conditions (\ref{Eq:BC_Bounds}) and (\ref{Eq:XC_Bounds}) as stated in Theorem~\ref{THM:Out_XC}, \emph{i.e.}
%\begin{subequations}
%\begin{align*}
%%\label{Eq:BC_Bounds}
%& \mathrm{BC~Bounds:~} \frac{R_{ij}}{1-\dl_{{\sf Tx}_j}} + \frac{R_{\bar{i}j} + R_{0j}}{1-\dl_{\bar{i}j}} \leq 1, \\
%%\label{Eq:XC_Bounds}
%& \mathrm{XC~Bounds:~} \frac{R_i}{1-\dl_{{\sf Tx}_j}} + \frac{R_{\bar{i}} + R_0}{1-\dl_{\bar{i}j}} \leq \frac{1-\dl_{{\sf Rx}_{\bar{i}}}}{1-\dl_{\bar{i}j}},
%\end{align*}
%\end{subequations}
%
%To achieve these rates, we follow the steps presented below.
%
%\noindent {\bf Step~1:~Multicast~Channel}: The capacity region of the two-user multicast channel is the intersection of the capacity regions of the two multiple-access channels formed at each receiver~\cite{AlirezaBFICDelayed}. Denote the rates corresponding to the maximum sum-rate point of this problem by $R^{\mathrm{MC}}_{1}$ and $R^{\mathrm{MC}}_{2}$. Note that $R^{\mathrm{MC}}_{i}$, $i=1,2$, is the overall rate intended for receiver $i$. Find $\gamma^{\mathrm{MC}}$ by solving
%\begin{align}
%& \max \gamma^{\mathrm{MC}} \nonumber \\
%& \text{s.t.}~R_{ii} \leq \gamma R^{\mathrm{IC}}_{i},~i=1,2.
%\end{align}
%Then, $\gamma^{\mathrm{IC}}$ denotes the fraction of time we deploy the achievability strategy of the two-user erasure IC with delayed CSIT given in~\cite{AlirezaBFICDelayed,vahid2016two}. During this portion of communications no interleaving is necessary.
%
%
%
%
%\noindent {\bf Step~2:~Interference~Channel}: The capacity region of the two-user erasure IC with delayed CSIT satisfying the conditions of Theorem~\ref{THM:Ach_XC} is given in~\cite{AlirezaBFICDelayed,vahid2016two}. Denote the rates corresponding to the maximum sum-rate point of this problem by $R^{\mathrm{IC}}_{1}$ and $R^{\mathrm{IC}}_{2}$. Note that $R^{\mathrm{IC}}_{i}$, $i=1,2$, is the communication rate between transmitter-receiver pair $i$. Find $\gamma^{\mathrm{IC}}$ by solving
%\begin{align}
%& \max \gamma^{\mathrm{IC}} \nonumber \\
%& \text{s.t.}~R_{ii} \leq \gamma R^{\mathrm{IC}}_{i},~i=1,2.
%\end{align}
%Then, $\gamma^{\mathrm{IC}}$ denotes the fraction of time we deploy the achievability strategy of the two-user erasure IC with delayed CSIT given in~\cite{AlirezaBFICDelayed,vahid2016two}. During this portion of communications no interleaving is necessary.
%
%
%\noindent {\bf Step~3:~Interference~Channel~with~swapped~IDs}: This step is very similar to previous one.  We treat the X-Channel as a two-user interference channel with swapped IDs in which ${\sf Tx}_i$ wishes to communicated with ${\sf Rx}_{\bar{i}}$, $i=1,2$, see Fig.~\ref{Fig:ExSymmetric}(c). Denote the rates corresponding to the maximum sum-rate point of this problem by $R^{\mathrm{ICS}}_{1}$ and $R^{\mathrm{ICS}}_{2}$. Note that $R^{\mathrm{ICS}}_{i}$, $i=1,2$, is the communication rate intended for receiver $i$ from transmitter $\bar{i}$. Find $\gamma^{\mathrm{ICS}}$ by solving
%\begin{align}
%& \max \gamma^{\mathrm{ICS}} \nonumber \\
%& \text{s.t.}~R_{i\bar{i}} \leq \gamma R^{\mathrm{ICS}}_{i},~i=1,2.
%\end{align}
%Then, $\gamma^{\mathrm{ICS}}$ denotes the fraction of time we deploy the achievability strategy of the two-user erasure IC with swapped IDs and delayed CSIT given in~\cite{AlirezaBFICDelayed,vahid2016two}. During this portion of communications no interleaving is necessary.
%
%\noindent {\bf Step~4:~Broadcast~Channel}:


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[ht]
\centering
\subfigure[]{\includegraphics[height = 2in]{FiguresPDF/Sub-Multicast-General.pdf}}
%
\subfigure[]{\includegraphics[height = 2in]{FiguresPDF/Sub-IC-General.pdf}}
%
\subfigure[]{\includegraphics[height = 2in]{FiguresPDF/Sub-ICSwapped-General.pdf}}
\caption{\it (a) The two-user multicast channel and its capacity region, the capacity can be achieved without using the delayed CSI; (b) The two-user binary fading interference channel and its capacity region; (c) The two-user binary fading interference channel with swapped IDs and its capacity region.\label{Fig:Gen}}
\end{figure}



The strategy that achieves the rates in (\ref{Eq:SymGeneral}) is similar to what we presented in Section~\ref{Section:Sym}. Define
\begin{align}
\label{Eq:gamma}
\gamma = \frac{R_0}{1-q^2}.
\end{align}

First, suppose 
\begin{align}
\frac{2\beta \left( 1-q^2\right)}{1+\beta} \leq 2p.
\end{align}
Then the transmission strategy is as follows.
\begin{itemize}

\item For the first $\gamma$ fraction of the communication block, we treat the X-Channel as a two-user multicast channel as depicted in Fig.~\ref{Fig:Gen}(a) in which each transmitter has a message for {\it both} receivers. For the two-user multicast channel with fading parameter $p$, the capacity region matches that of the multiple-access channel formed at each receiver~\cite{AlirezaBFICDelayed} and depicted in Fig.~\ref{Fig:Gen}(a) as well.

\item During a fraction $(1-\gamma)/2$ of the communication block, we treat the X-Channel as a two-user interference channel in which ${\sf Tx}_j$ wishes to communicated with ${\sf Rx}_j$, see Fig.~\ref{Fig:Gen}(b). An instance of the capacity region of this problem is given in~\cite{AlirezaBFICDelayed} and depicted in Fig.~\ref{Fig:Gen}(b).

\item During a fraction $(1-\gamma)/2$ of the communication block, we treat the X-Channel as a two-user interference channel with swapped IDs in which ${\sf Tx}_j$ wishes to communicated with ${\sf Rx}_{\bar{j}}$, see Fig.~\ref{Fig:Gen}(c). In the homogeneous setting of this work, the capacity region of this interference channel with swapped IDs matches that of the previous case and an instance of it is depicted in Fig.~\ref{Fig:Gen}(c).

\end{itemize}

\noindent {\bf Achievable Rates}: With this strategy $\gamma$ fraction of the times, we achieve a common rate of $\left( 1 - q^2 \right)$, while $(1-\gamma)$ fraction of the times, we achieve individual rates
\begin{align}
\left( \frac{\beta \left( 1-q^2\right)}{1+\beta}, \frac{\beta \left( 1-q^2\right)}{1+\beta} \right).
\end{align}
The overall achievable rate matches $\mathcal{C}_{\sf SUM}\left( R_0 \right)$ in this case. Now, consider the case in which
\begin{align}
\frac{2\beta \left( 1-q^2\right)}{1+\beta} > 2p.
\end{align}
We need to modify the strategy slightly. The transmission strategy for the interference channel consists of two phases. During Phase~1, uncoded bits intended for different receivers are transmitted. During Phases~2, using the delayed CSIT, the previously transmitted bits are combined and repackaged to create bits of common interest. These bits are then transmitted using the capacity-achieving strategy of the multicast problem. In the modified strategy for the X-Channel, Phase~1 consists of two sub-phases. In the first sub-phase, both transmitters send out bits intended for ${\sf Rx}_1$ while in the second sub-phases, bits intended for ${\sf Rx}_2$ are communicated. This way we take full advantage of the entire signal space at each receiver and the individual rates are no longer limited by the capacity of a point-to-point channel. The second phase is identical to the Interference Channel.  

\begin{figure}[ht]
\centering
\includegraphics[height = 2in]{FiguresPDF/Sub-MAC-General.pdf}
\caption{\it The multiple-access channel formed at ${\sf Rx}_1$ and its capacity region.\label{Fig:MAC}}
\end{figure}

{\color{blue} \subsection{Transmission Strategy: Other Corner Points}
\label{Section:Other}

% {\color{red} Alireza, discuss one that XC bounds are tight first.}

As mentioned earlier, for the homogeneous setting we consider in this work, the maximum sum-rate is attained when all $R_{ij}$'s are equal, $i,j \in \{ 1, 2\}$. Achieving unequal rates for different users follows the same logic with careful application of sub-problems as illustrated in Section~\ref{Section:Unequal}. Here, we provide a detailed description of the achievability of such corner points. To simplify the argument, we first assume $R_0 = 0$, \emph{i.e.} no common rate, and later explain how the strategy changes when common rate is non-zero.

The capacity region as described in Theorem~\ref{THM:Out_XC} is defined by the following six bounds:
\begin{equation}
\label{Eq:AchBC1}
\mathrm{BC~at~} {\sf Tx}_1:~\left\{ \begin{array}{ll}
\vspace{1mm}\mathrm{(a)}~0 \leq R_{11} + \beta \left( R_{21} + R_{01} \right) \leq \beta p, & \\
\mathrm{(b)}~0 \leq R_{21} + \beta \left( R_{11} + R_{01} \right) \leq \beta p, & 
\end{array} \right.
\end{equation}
\begin{equation}
\label{Eq:AchBC2}
\mathrm{BC~at~} {\sf Tx}_2:~\left\{ \begin{array}{ll}
\vspace{1mm}\mathrm{(a)}~0 \leq R_{12} + \beta \left( R_{22} + R_{02} \right) \leq \beta p, & \\
\mathrm{(b)}~0 \leq R_{22} + \beta \left( R_{12} + R_{02} \right) \leq \beta p, & 
\end{array} \right.
\end{equation}
\begin{equation}
\label{Eq:AchXC}
\mathrm{XC~Bounds}:~\left\{ \begin{array}{ll}
\vspace{1mm}\mathrm{(a)}~R_1 + \beta \left( R_{2} + R_0 \right) \leq \beta \left( 1 - q^2 \right), & \\
\mathrm{(b)}~\beta \left( R_{1} + R_0 \right) + R_2 \leq \beta \left( 1 - q^2 \right), & 
\end{array} \right.
\end{equation}
where $R_1 = R_{11} + R_{12}$ and $R_2 = R_{21} + R_{22}$.

We start by assuming the BC bounds at ${\sf Tx}_1$ are tight. By symmetry, this also covers the BC bounds at ${\sf Tx}_2$ being tight. We need to cover the following cases which correspond to the different corner points of the BC formed at ${\sf Tx}_1$:
\begin{itemize}

\item Case (a): In this case, $R_{11} = p$, which from \eqref{Eq:AchBC1}(b) results in $R_{21}  = 0$. Then, from \eqref{Eq:AchXC}(b), maximizing $R_1$ gives us $R_{12} = p(1-p)$ and $R_{22} = 0$. A closer look reveals that this is the capacity region of the MAC formed at ${\sf Rx}_1$ foe which the achievability is straightforward. As an example, for $p = 0.5$, corner point
\begin{align}
\left( R_0, R_1, R_2 \right) = \left( 0, 3/4, 0 \right)
\end{align}
of Fig.~\ref{Fig:CommonRates}(a) falls in this category. This corner point corresponds to the Multiple-Access Channel formed at ${\sf Rx}_1$ as depicted in Fig.~\ref{Fig:MAC}. 

\item Case (b): In this case, we consider the maximum sum-rate point for the BC formed at ${\sf Tx}_1$, which gives us
\begin{align}
\label{Eq:Casebbreak}
R_{11} = R_{21} = \frac{\beta p}{1+\beta}.
\end{align}
To maximize $R_1$, we set $R_{22} = 0$, and from \eqref{Eq:AchXC}(b), we get
\begin{align}
R_1 = \frac{\beta(1-q^2)-R_{21}}{\beta},% \frac{\beta^3 p}{1+\beta},
\end{align}
and since $R_1 = R_{11} + R_{12}$, we obtain
\begin{align}
R_{12} = R_1 - R_{11} = p(1-p).% \frac{\beta^3 p}{1+\beta} - \frac{\beta p}{1+\beta} = \beta p(1-p).
\end{align}
To summarize the discussion above, since we are assuming $R_0 = 0$ in this case, we have
\begin{align}
\label{eq:cornornocommon}
% \left( R_{11}, R_{12}, R_{21}, R_{22} \right) = \left( \frac{\beta p}{1+\beta}, \beta p(1-p), \frac{\beta p}{1+\beta}, 0 \right).
\left( R_{11}, R_{12}, R_{21}, R_{22} \right) = \left( \frac{\beta p}{1+\beta}, p(1-p), \frac{\beta p}{1+\beta}, 0 \right).
\end{align}
This corner point is then achievable by using the maximum achievable sum-rate strategy for the BC at transmitter ${\sf Tx}_1$. Simultaneously, ${\sf Tx}_2$ encodes $W_{12}$ using an erasure code at rate $p(1-p)$. Each receiver first decodes $W_{12}$ treating the signal from ${\sf Tx}_1$ as noise. We note that  $W_{12}$ is not needed at ${\sf Rx}_2$, but due to the associated rate, $p(1-p)$, the second receiver can decode this message. After decoding $W_{12}$ and removing its contribution from the received signal, the remaining strategy is identical to that of the maximum sum-rate point of the BC at transmitter ${\sf Tx}_1$, and thus, the proof for \eqref{eq:cornornocommon} is complete. 
%This corner point is then achievable by using the maximum achievable sum-rate strategy for IC with swapped ID of Fig.~\ref{Fig:ExSymmetric}(c) for a fraction $p$ of the communication time, and the achievability strategy of the MAC at ${\sf Rx}_1$ similar to Fig.~\ref{Fig:MAC} for a fraction $(1-p)$ of the communication time. This follows from
%\begin{align}
%R_{11} + R_{12} - R_{21} = \frac{\beta p}{1+\beta} + \frac{\beta p (\beta^2 - 2)}{1+\beta} = \underbrace{(\beta - 1)}_{=~(1-p)} \underbrace{\beta p}_{\text{MAC~at~}{\sf Rx}_1}.
%\end{align}  
After \eqref{Eq:Casebbreak}, we chose to maximize $R_1$ through the XC bound of  \eqref{Eq:AchXC}(a), maximizing $R_2$ would have resulted in $R_{12} = 0$ and $R_{22} = \beta p(1-p)$, and the achievability would have been similar. 

\end{itemize}

So far, we covered the case in which the BC bounds at one transmitter are tight. Other corner points may also result from having a mixture of outer-bounds being tight but not necessarily at each transmitter. For instance, we could have outer-bound of \eqref{Eq:AchBC1}(a) and \eqref{Eq:AchBC2}(a) active. The corner points that are obtained this way, as described below, will be similar to what we have already covered. The extreme point of \eqref{Eq:AchBC1}(a), \emph{i.e.} $R_{21} = p$ and $R_{11} = 0$, will follow similar steps to Case (a) above with rearranging IDs. So, let's consider the less trivial case in which   
\begin{align}
R_{11} = R_{21} = \frac{\beta p}{1+\beta},
\end{align} 
similar to \eqref{Eq:Casebbreak}. The next step is to maximize either $R_1$ through \eqref{Eq:AchXC}(a) or $R_2$ through \eqref{Eq:AchXC}(b), and in conjunction with \eqref{Eq:AchBC2}(a), deducing $R_{12}$ and $R_{22}$. However, this is similar to Case (b) above and the achievability follows. 
 
The final step in completing the achievability strategy is to discuss how to handle the common rate. The details are similar to what we have covered for $R_0 = 0$, and thus, we only highlight the differences. As in the case of BCs with common rate~\cite{georgiadis2009broadcast,Vahid-BCCommon}, having homogeneous channel parameters simplifies the strategy. To handle the common rate, the first step is to deliver $\min \{ R_{01}, R_{02} \}$ using the transmission strategy of the multicast problem of  Fig.~\ref{Fig:ExSymmetric}(a). The next steps will follows from using IC and IC with swapped IDs to deliver private messages. Finally, the remaining common rate at one of the transmitters, will be delivered through the strategy of BCs with common rate, and simultaneously, the other transmitter communicates its messages. 
 
In summary, in this section, we presented the transmission strategy for $\mathcal{C}_{\sf SUM}\left( R_0 \right)$ where $0 \leq R_0 \leq (1-q^2)$. We also discussed and highlighted the strategy for other corner points of the capacity region. This completes the proof of Theorem~\ref{THM:Out_XC}.}


==> Camera Ready/Achievability_XC.tex <==
X-Channels can be thought of as a generalization of several known problems such as interference channels, broadcast channels, multiple-access channels, and multicast channels. In the previous section, we developed a set of new outer-bounds for this problem. In this section, we show that a careful combination of the capacity-achieving strategies for other known known problems will achieve the capacity region of the X-Channel. However, in Section~\ref{Section:Gen}, we show that if we treat the X-Channel as a number of disjoint sub-problems, we may not achieve the capacity. In fact, in some regimes, we need to interleave the capacity-achieving strategies of different sub-problems and execute them simultaneously.

To describe the transmission strategy, we first present two examples. The first example describes a symmetric scenario associated with Fig.~\ref{Fig:CommonRates}(b), and the second example describes a scenario in which transmitters achieve unequal rates. After the examples, we present the general scheme.

\begin{figure}[ht]
\centering
\subfigure[]{\includegraphics[height = 2in]{FiguresPDF/Sub-Multicast.pdf}}
%
\subfigure[]{\includegraphics[height = 2in]{FiguresPDF/Sub-IC.pdf}}
%
\subfigure[]{\includegraphics[height = 2in]{FiguresPDF/Sub-ICSwapped.pdf}}
\caption{\it (a) The two-user multicast channel and its capacity region, the capacity can be achieved without using the delayed CSI; (b) The two-user binary fading interference channel and its capacity region; (c) The two-user binary fading interference channel with swapped IDs and its capacity region.\label{Fig:ExSymmetric}}
\end{figure}

\subsection{Example~1:~Symmetric Sum-Rate of Fig.~\ref{Fig:CommonRates}(b)}
\label{Section:Sym}

Suppose for $p = 0.5$, we wish to achieve the sum-capacity of $\mathcal{C}_{\sf SUM}\left( 1/4 \right) = 0.85$, as defined in (\ref{Eq:CSUM}), with
\begin{align}
\label{Eq:RatesEx1}
& R_{01} = R_{02} = 1/8, \nonumber \\
& R_{11} = R_{12} = R_{21} = R_{22} = 0.15,
\end{align}
as shown in Fig.~\ref{Fig:CommonRates}(b). 

For this particular example, we treat the X-Channel as three separate problems listed below at different times, and we show that this strategy achieves the capacity.
\begin{itemize}

\item For the first third of the communication block, we treat the X-Channel as a two-user multicast channel as depicted in Fig.~\ref{Fig:ExSymmetric}(a) in which each transmitter has a message for {\it both} receivers. For the two-user multicast channel with fading parameter $1/2$, the capacity region matches that of the multiple-access channel formed at each receiver~\cite{AlirezaBFICDelayed} and depicted in Fig.~\ref{Fig:ExSymmetric}(a) as well.

\item For the second third of the communication block, we treat the X-Channel as a two-user interference channel in which ${\sf Tx}_j$ wishes to communicated with ${\sf Rx}_j$, see Fig.~\ref{Fig:ExSymmetric}(b). The capacity region of this problem is given in~\cite{AlirezaBFICDelayed} and depicted in Fig.~\ref{Fig:ExSymmetric}(b).

\item During the final third of the communication block, we treat the X-Channel as a two-user interference channel with swapped IDs in which ${\sf Tx}_j$ wishes to communicated with ${\sf Rx}_{\bar{j}}$, see Fig.~\ref{Fig:ExSymmetric}(c). In the homogeneous setting of this work, the capacity region of this interference channel with swapped IDs matches that of the previous case and is depicted in Fig.~\ref{Fig:ExSymmetric}(c).

\end{itemize}

\noindent {\bf Achievable Rates}: We note that as the communication block length, $n$, goes to infinity, so do the communication block lengths for each sub-problem. Thus, during the first third of the communication block, we can achieve symmetric common rates arbitrary close to $\left( 3/8, 3/8 \right)$. Normalizing to the total communication block, we achieve $\left( R_{01}, R_{02} \right) = \left( 1/8, 1/8 \right)$ which matches the requirements of (\ref{Eq:RatesEx1}). From~\cite{AlirezaBFICDelayed} we know that for the two-user binary fading interference channel with delayed CSIT and $p =1/2$, we can achieve symmetric rates of $\left( 0.45, 0.45 \right)$. Normalizing to the total communication block, we achieve $\left( R_{11}, R_{22} \right) = \left( 0.15, 0.15 \right)$ which matches the requirements of (\ref{Eq:RatesEx1}). Finally, during  the final third of the communication block we treat the problem as a two-user interference channel with swapped IDs in which we can achieve symmetric rates of $\left( 0.45, 0.45 \right)$. Normalizing to the total communication block, we achieve $\left( R_{21}, R_{12} \right) = \left( 0.15, 0.15 \right)$ which again matches the requirements of (\ref{Eq:RatesEx1}). Thus, with splitting up the X-Channel into a combination of three known sub-problems, we can achieve the outer-bound region described in Theorem~\ref{THM:Out_XC}.

\begin{figure}[ht]
\centering
\subfigure[]{\includegraphics[height = 1.5in]{FiguresPDF/Sub-BCCommon.pdf}}
%
\subfigure[]{\includegraphics[height = 2in]{FiguresPDF/Sub-BCDelayed.pdf}}
\caption{\it (a) The two-user broadcast channel with a single common message; (b) The two-user broadcast channel with delayed CSIT and private messages, and its capacity region.\label{Fig:ExUnequal}}
\end{figure}


\subsection{Example~2:~Unequal Rates}
\label{Section:Unequal}

In the previous subsection we focused on a symmetric setting. Here, we discuss a scenario in which transmitters have different types of messages with different rates for each receiver. More precisely, we consider the region in Fig.~\ref{Fig:CommonRates}(c) for $p = 0.5$, and
\begin{align}
\label{Eq:RatesEx2}
& R_{01} = 1/2, \nonumber \\
& R_{02} = 0, \nonumber \\
& R_{11} = R_{21} = 0, \nonumber \\
& R_{12} = R_{22} = 0.15,
\end{align}

In this case, we can think of the X-Channel in this case as two sub-problems that coexist at the same time as described below.
\begin{itemize}

\item The Binary Fading Broadcast Channel from ${\sf Tx}_1$ as in Fig.~\ref{Fig:ExUnequal}(a) in which a single message is intended for both receivers. For this problem, the capacity can be achieved using a point-to-point erasure code of rate $1/2$.

\item The Binary Fading Broadcast Channel from ${\sf Tx}_2$ as in Fig.~\ref{Fig:ExUnequal}(b) with delayed CSIT in which the transmitter has a private message for each receiver. For this problem, the capacity region is given in~\cite{jolfaei1993new,georgiadis2009broadcast} and depicted Fig.~\ref{Fig:ExUnequal}(b). As described below, in order to be able to decode the messages in the presence of the broadcast channel from ${\sf Tx}_1$, we first encode $W_{12}$ and $W_{22}$ using point-to-point erasure codes of rate $1/2$, and treat the resulting codes as the input messages to the broadcast channel of Fig.~\ref{Fig:ExUnequal}(b).   

\end{itemize}

\noindent {\bf Achievable Rates}: At each receiver the received signal from ${\sf Tx}_2$ is corrupted (erased) half of times by the signal from ${\sf Tx}_1$. As a result, when we implement the capacity-achieving strategy of~\cite{jolfaei1993new,georgiadis2009broadcast}, we only deliver half of the bits intended for each receiver. However, since we first encode $W_{12}$ and $W_{22}$ using point-to-point erasure codes of rate $1/2$, obtaining half of the bits is sufficient for reliable decoding of $W_{12}$ and $W_{22}$. Thus, we achieve
\begin{align}
\left( R_{12}, R_{22} \right) = \frac{1}{2} \left( 0.3, 0.3 \right) = \left( 0.15, 0.15 \right), 
\end{align}
which again matches the requirements of (\ref{Eq:RatesEx2}). At the end of the communication block, receivers decode $W_{12}$ and $W_{22}$, and remove the contribution of ${\sf Tx}_2$ from their received signals. After removing the contribution of $X_2^n$, the problem is identical to the broadcast channel from ${\sf Tx}_1$ as in Fig.~\ref{Fig:ExUnequal}(a) for which we can achieve a common rate $R_{02}$ of $1/2$. 


\subsection{A Note on the X-Channel vs. the Interference Channel}
\label{Section:XCvsIC}


\begin{figure}[ht]
\centering
\includegraphics[height = 3in]{FiguresPDF/SumCapacity.pdf}
\caption{\it The sum-capacity of the X-Channel vs. that of the Interference Channel. To have a fair comparison, in the X-Channel we set $R_0 = 0$.\label{Fig:SumCapacity}}
\end{figure}


An important difference between the X-Channel and the interference channel is the fact that in the latter scenario, the individual rates are limited by the capacity of a point-to-point channel, \emph{i.e.} $p$. As a result, for the interference channel, we have~\cite{AlirezaBFICDelayed}:
\begin{align} 
\text{Interference~Channel:~}\sup{\left( R_1+R_2 \right)} = \min\left\{  2p, \frac{2\beta \left( 1-q^2\right)}{1+\beta} \right\}.
\end{align}
However, in the X-Channel no such limitation exists, and we have
\begin{align} 
\text{X-Channel:~}\sup{\left(R_1+R_2\right)} = \frac{2\beta \left\{ \left( 1-q^2\right) - R_0 \right\}}{1+\beta}.
\end{align}  
The difference is depicted in Fig.~\ref{Fig:SumCapacity} for $R_0 = 0$. This means that if we naively try to use the capacity-achieving strategies of the sub-problems independently, we cannot achieve the capacity region of the X-Channel. The key idea to overcome this challenge is to take an approach similar to the one we presented in Section~\ref{Section:Unequal} and run different strategies simultaneously as described below. 


\subsection{Transmission Strategy: Maximum Symmetric Point}
\label{Section:Gen}

The two examples we have provided so far demonstrate the key ideas behind the transmission strategy. We now present a systematic way of utilizing the capacity-achieving strategies of other problems, such as the interference channel and the multicast channel, in order to achieve the capacity region of the X-Channel. % As mentioned before, our results rely on the achievability strategy of other well-known problems, including the two-user erasure interference channel with delayed CSIT. Since the capacity region of this latter problem is only known for the conditions of Theorem~\ref{THM:Ach_XC}, we could not achieve the outer-bound region of Theorem~\ref{THM:Out_XC} for all values of erasure probabilities.

Fix $0 \leq R_0 \leq (1-q^2)$. Then, our goal is the maximum sum-rate point derived from the outer-bounds of Theorem~\ref{THM:Out_XC}. In other words, we need to achieve
\begin{align}
\label{Eq:SymGeneral}
& 0 \leq R_0 \leq (1-q^2), \nonumber \\
& R_1 = R_2 = \frac{\beta \left[ (1-q^2) - R_0 \right]}{1+\beta}.
\end{align}
For the homogeneous setting that we consider in this work, the maximum sum-rate is attained when all $R_{ij}$'s are equal, $i,j \in \{ 1, 2\}$. We first focus on this maximum sum-rate corner point. % and all other corner points are achieved by tuning the 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%Fix $(R_{01},R_{02},R_{11},R_{12},R_{21},R_{22})$ satisfying conditions (\ref{Eq:BC_Bounds}) and (\ref{Eq:XC_Bounds}) as stated in Theorem~\ref{THM:Out_XC}, \emph{i.e.}
%\begin{subequations}
%\begin{align*}
%%\label{Eq:BC_Bounds}
%& \mathrm{BC~Bounds:~} \frac{R_{ij}}{1-\dl_{{\sf Tx}_j}} + \frac{R_{\bar{i}j} + R_{0j}}{1-\dl_{\bar{i}j}} \leq 1, \\
%%\label{Eq:XC_Bounds}
%& \mathrm{XC~Bounds:~} \frac{R_i}{1-\dl_{{\sf Tx}_j}} + \frac{R_{\bar{i}} + R_0}{1-\dl_{\bar{i}j}} \leq \frac{1-\dl_{{\sf Rx}_{\bar{i}}}}{1-\dl_{\bar{i}j}},
%\end{align*}
%\end{subequations}
%
%To achieve these rates, we follow the steps presented below.
%
%\noindent {\bf Step~1:~Multicast~Channel}: The capacity region of the two-user multicast channel is the intersection of the capacity regions of the two multiple-access channels formed at each receiver~\cite{AlirezaBFICDelayed}. Denote the rates corresponding to the maximum sum-rate point of this problem by $R^{\mathrm{MC}}_{1}$ and $R^{\mathrm{MC}}_{2}$. Note that $R^{\mathrm{MC}}_{i}$, $i=1,2$, is the overall rate intended for receiver $i$. Find $\gamma^{\mathrm{MC}}$ by solving
%\begin{align}
%& \max \gamma^{\mathrm{MC}} \nonumber \\
%& \text{s.t.}~R_{ii} \leq \gamma R^{\mathrm{IC}}_{i},~i=1,2.
%\end{align}
%Then, $\gamma^{\mathrm{IC}}$ denotes the fraction of time we deploy the achievability strategy of the two-user erasure IC with delayed CSIT given in~\cite{AlirezaBFICDelayed,vahid2016two}. During this portion of communications no interleaving is necessary.
%
%
%
%
%\noindent {\bf Step~2:~Interference~Channel}: The capacity region of the two-user erasure IC with delayed CSIT satisfying the conditions of Theorem~\ref{THM:Ach_XC} is given in~\cite{AlirezaBFICDelayed,vahid2016two}. Denote the rates corresponding to the maximum sum-rate point of this problem by $R^{\mathrm{IC}}_{1}$ and $R^{\mathrm{IC}}_{2}$. Note that $R^{\mathrm{IC}}_{i}$, $i=1,2$, is the communication rate between transmitter-receiver pair $i$. Find $\gamma^{\mathrm{IC}}$ by solving
%\begin{align}
%& \max \gamma^{\mathrm{IC}} \nonumber \\
%& \text{s.t.}~R_{ii} \leq \gamma R^{\mathrm{IC}}_{i},~i=1,2.
%\end{align}
%Then, $\gamma^{\mathrm{IC}}$ denotes the fraction of time we deploy the achievability strategy of the two-user erasure IC with delayed CSIT given in~\cite{AlirezaBFICDelayed,vahid2016two}. During this portion of communications no interleaving is necessary.
%
%
%\noindent {\bf Step~3:~Interference~Channel~with~swapped~IDs}: This step is very similar to previous one.  We treat the X-Channel as a two-user interference channel with swapped IDs in which ${\sf Tx}_i$ wishes to communicated with ${\sf Rx}_{\bar{i}}$, $i=1,2$, see Fig.~\ref{Fig:ExSymmetric}(c). Denote the rates corresponding to the maximum sum-rate point of this problem by $R^{\mathrm{ICS}}_{1}$ and $R^{\mathrm{ICS}}_{2}$. Note that $R^{\mathrm{ICS}}_{i}$, $i=1,2$, is the communication rate intended for receiver $i$ from transmitter $\bar{i}$. Find $\gamma^{\mathrm{ICS}}$ by solving
%\begin{align}
%& \max \gamma^{\mathrm{ICS}} \nonumber \\
%& \text{s.t.}~R_{i\bar{i}} \leq \gamma R^{\mathrm{ICS}}_{i},~i=1,2.
%\end{align}
%Then, $\gamma^{\mathrm{ICS}}$ denotes the fraction of time we deploy the achievability strategy of the two-user erasure IC with swapped IDs and delayed CSIT given in~\cite{AlirezaBFICDelayed,vahid2016two}. During this portion of communications no interleaving is necessary.
%
%\noindent {\bf Step~4:~Broadcast~Channel}:


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[ht]
\centering
\subfigure[]{\includegraphics[height = 2in]{FiguresPDF/Sub-Multicast-General.pdf}}
%
\subfigure[]{\includegraphics[height = 2in]{FiguresPDF/Sub-IC-General.pdf}}
%
\subfigure[]{\includegraphics[height = 2in]{FiguresPDF/Sub-ICSwapped-General.pdf}}
\caption{\it (a) The two-user multicast channel and its capacity region, the capacity can be achieved without using the delayed CSI; (b) The two-user binary fading interference channel and its capacity region; (c) The two-user binary fading interference channel with swapped IDs and its capacity region.\label{Fig:Gen}}
\end{figure}



The strategy that achieves the rates in (\ref{Eq:SymGeneral}) is similar to what we presented in Section~\ref{Section:Sym}. Define
\begin{align}
\label{Eq:gamma}
\gamma = \frac{R_0}{1-q^2}.
\end{align}

First, suppose 
\begin{align}
\frac{2\beta \left( 1-q^2\right)}{1+\beta} \leq 2p.
\end{align}
Then the transmission strategy is as follows.
\begin{itemize}

\item For the first $\gamma$ fraction of the communication block, we treat the X-Channel as a two-user multicast channel as depicted in Fig.~\ref{Fig:Gen}(a) in which each transmitter has a message for {\it both} receivers. For the two-user multicast channel with fading parameter $p$, the capacity region matches that of the multiple-access channel formed at each receiver~\cite{AlirezaBFICDelayed} and depicted in Fig.~\ref{Fig:Gen}(a) as well.

\item During a fraction $(1-\gamma)/2$ of the communication block, we treat the X-Channel as a two-user interference channel in which ${\sf Tx}_j$ wishes to communicated with ${\sf Rx}_j$, see Fig.~\ref{Fig:Gen}(b). An instance of the capacity region of this problem is given in~\cite{AlirezaBFICDelayed} and depicted in Fig.~\ref{Fig:Gen}(b).

\item During a fraction $(1-\gamma)/2$ of the communication block, we treat the X-Channel as a two-user interference channel with swapped IDs in which ${\sf Tx}_j$ wishes to communicated with ${\sf Rx}_{\bar{j}}$, see Fig.~\ref{Fig:Gen}(c). In the homogeneous setting of this work, the capacity region of this interference channel with swapped IDs matches that of the previous case and an instance of it is depicted in Fig.~\ref{Fig:Gen}(c).

\end{itemize}

\noindent {\bf Achievable Rates}: With this strategy $\gamma$ fraction of the times, we achieve a common rate of $\left( 1 - q^2 \right)$, while $(1-\gamma)$ fraction of the times, we achieve individual rates
\begin{align}
\left( \frac{\beta \left( 1-q^2\right)}{1+\beta}, \frac{\beta \left( 1-q^2\right)}{1+\beta} \right).
\end{align}
The overall achievable rate matches $\mathcal{C}_{\sf SUM}\left( R_0 \right)$ in this case. Now, consider the case in which
\begin{align}
\frac{2\beta \left( 1-q^2\right)}{1+\beta} > 2p.
\end{align}
We need to modify the strategy slightly. The transmission strategy for the interference channel consists of two phases. During Phase~1, uncoded bits intended for different receivers are transmitted. During Phases~2, using the delayed CSIT, the previously transmitted bits are combined and repackaged to create bits of common interest. These bits are then transmitted using the capacity-achieving strategy of the multicast problem. In the modified strategy for the X-Channel, Phase~1 consists of two sub-phases. In the first sub-phase, both transmitters send out bits intended for ${\sf Rx}_1$ while in the second sub-phases, bits intended for ${\sf Rx}_2$ are communicated. This way we take full advantage of the entire signal space at each receiver and the individual rates are no longer limited by the capacity of a point-to-point channel. The second phase is identical to the Interference Channel.  

\begin{figure}[ht]
\centering
\includegraphics[height = 2in]{FiguresPDF/Sub-MAC-General.pdf}
\caption{\it The multiple-access channel formed at ${\sf Rx}_1$ and its capacity region.\label{Fig:MAC}}
\end{figure}

{\color{blue} \subsection{Transmission Strategy: Other Corner Points}
\label{Section:Other}

% {\color{red} Alireza, discuss one that XC bounds are tight first.}

As mentioned earlier, for the homogeneous setting we consider in this work, the maximum sum-rate is attained when all $R_{ij}$'s are equal, $i,j \in \{ 1, 2\}$. Achieving unequal rates for different users follows the same logic with careful application of sub-problems as illustrated in Section~\ref{Section:Unequal}. Here, we provide a detailed description of the achievability of such corner points. To simplify the argument, we first assume $R_0 = 0$, \emph{i.e.} no common rate, and later explain how the strategy changes when common rate is non-zero.

The capacity region as described in Theorem~\ref{THM:Out_XC} is defined by the following six bounds:
\begin{equation}
\label{Eq:AchBC1}
\mathrm{BC~at~} {\sf Tx}_1:~\left\{ \begin{array}{ll}
\vspace{1mm}\mathrm{(a)}~0 \leq R_{11} + \beta \left( R_{21} + R_{01} \right) \leq \beta p, & \\
\mathrm{(b)}~0 \leq R_{21} + \beta \left( R_{11} + R_{01} \right) \leq \beta p, & 
\end{array} \right.
\end{equation}
\begin{equation}
\label{Eq:AchBC2}
\mathrm{BC~at~} {\sf Tx}_2:~\left\{ \begin{array}{ll}
\vspace{1mm}\mathrm{(a)}~0 \leq R_{12} + \beta \left( R_{22} + R_{02} \right) \leq \beta p, & \\
\mathrm{(b)}~0 \leq R_{22} + \beta \left( R_{12} + R_{02} \right) \leq \beta p, & 
\end{array} \right.
\end{equation}
\begin{equation}
\label{Eq:AchXC}
\mathrm{XC~Bounds}:~\left\{ \begin{array}{ll}
\vspace{1mm}\mathrm{(a)}~R_1 + \beta \left( R_{2} + R_0 \right) \leq \beta \left( 1 - q^2 \right), & \\
\mathrm{(b)}~\beta \left( R_{1} + R_0 \right) + R_2 \leq \beta \left( 1 - q^2 \right), & 
\end{array} \right.
\end{equation}
where $R_1 = R_{11} + R_{12}$ and $R_2 = R_{21} + R_{22}$.

We start by assuming the BC bounds at ${\sf Tx}_1$ are tight. By symmetry, this also covers the BC bounds at ${\sf Tx}_2$ being tight. We need to cover the following cases which correspond to the different corner points of the BC formed at ${\sf Tx}_1$:
\begin{itemize}

\item Case (a): In this case, $R_{11} = p$, which from \eqref{Eq:AchBC1}(b) results in $R_{21}  = 0$. Then, from \eqref{Eq:AchXC}(b), maximizing $R_1$ gives us $R_{12} = p(1-p)$ and $R_{22} = 0$. A closer look reveals that this is the capacity region of the MAC formed at ${\sf Rx}_1$ foe which the achievability is straightforward. As an example, for $p = 0.5$, corner point
\begin{align}
\left( R_0, R_1, R_2 \right) = \left( 0, 3/4, 0 \right)
\end{align}
of Fig.~\ref{Fig:CommonRates}(a) falls in this category. This corner point corresponds to the Multiple-Access Channel formed at ${\sf Rx}_1$ as depicted in Fig.~\ref{Fig:MAC}. 

\item Case (b): In this case, we consider the maximum sum-rate point for the BC formed at ${\sf Tx}_1$, which gives us
\begin{align}
\label{Eq:Casebbreak}
R_{11} = R_{21} = \frac{\beta p}{1+\beta}.
\end{align}
To maximize $R_1$, we set $R_{22} = 0$, and from \eqref{Eq:AchXC}(b), we get
\begin{align}
R_1 = \frac{\beta(1-q^2)-R_{21}}{\beta},% \frac{\beta^3 p}{1+\beta},
\end{align}
and since $R_1 = R_{11} + R_{12}$, we obtain
\begin{align}
R_{12} = R_1 - R_{11} = p(1-p).% \frac{\beta^3 p}{1+\beta} - \frac{\beta p}{1+\beta} = \beta p(1-p).
\end{align}
To summarize the discussion above, since we are assuming $R_0 = 0$ in this case, we have
\begin{align}
\label{eq:cornornocommon}
% \left( R_{11}, R_{12}, R_{21}, R_{22} \right) = \left( \frac{\beta p}{1+\beta}, \beta p(1-p), \frac{\beta p}{1+\beta}, 0 \right).
\left( R_{11}, R_{12}, R_{21}, R_{22} \right) = \left( \frac{\beta p}{1+\beta}, p(1-p), \frac{\beta p}{1+\beta}, 0 \right).
\end{align}
This corner point is then achievable by using the maximum achievable sum-rate strategy for the BC at transmitter ${\sf Tx}_1$. Simultaneously, ${\sf Tx}_2$ encodes $W_{12}$ using an erasure code at rate $p(1-p)$. Each receiver first decodes $W_{12}$ treating the signal from ${\sf Tx}_1$ as noise. We note that  $W_{12}$ is not needed at ${\sf Rx}_2$, but due to the associated rate, $p(1-p)$, the second receiver can decode this message. After decoding $W_{12}$ and removing its contribution from the received signal, the remaining strategy is identical to that of the maximum sum-rate point of the BC at transmitter ${\sf Tx}_1$, and thus, the proof for \eqref{eq:cornornocommon} is complete. 
%This corner point is then achievable by using the maximum achievable sum-rate strategy for IC with swapped ID of Fig.~\ref{Fig:ExSymmetric}(c) for a fraction $p$ of the communication time, and the achievability strategy of the MAC at ${\sf Rx}_1$ similar to Fig.~\ref{Fig:MAC} for a fraction $(1-p)$ of the communication time. This follows from
%\begin{align}
%R_{11} + R_{12} - R_{21} = \frac{\beta p}{1+\beta} + \frac{\beta p (\beta^2 - 2)}{1+\beta} = \underbrace{(\beta - 1)}_{=~(1-p)} \underbrace{\beta p}_{\text{MAC~at~}{\sf Rx}_1}.
%\end{align}  
After \eqref{Eq:Casebbreak}, we chose to maximize $R_1$ through the XC bound of  \eqref{Eq:AchXC}(a), maximizing $R_2$ would have resulted in $R_{12} = 0$ and $R_{22} = \beta p(1-p)$, and the achievability would have been similar. 

\end{itemize}

So far, we covered the case in which the BC bounds at one transmitter are tight. Other corner points may also result from having a mixture of outer-bounds being tight but not necessarily at each transmitter. For instance, we could have outer-bound of \eqref{Eq:AchBC1}(a) and \eqref{Eq:AchBC2}(a) active. The corner points that are obtained this way, as described below, will be similar to what we have already covered. The extreme point of \eqref{Eq:AchBC1}(a), \emph{i.e.} $R_{21} = p$ and $R_{11} = 0$, will follow similar steps to Case (a) above with rearranging IDs. So, let's consider the less trivial case in which   
\begin{align}
R_{11} = R_{21} = \frac{\beta p}{1+\beta},
\end{align} 
similar to \eqref{Eq:Casebbreak}. The next step is to maximize either $R_1$ through \eqref{Eq:AchXC}(a) or $R_2$ through \eqref{Eq:AchXC}(b), and in conjunction with \eqref{Eq:AchBC2}(a), deducing $R_{12}$ and $R_{22}$. However, this is similar to Case (b) above and the achievability follows. 
 
The final step in completing the achievability strategy is to discuss how to handle the common rate. The details are similar to what we have covered for $R_0 = 0$, and thus, we only highlight the differences. As in the case of BCs with common rate~\cite{georgiadis2009broadcast,Vahid-BCCommon}, having homogeneous channel parameters simplifies the strategy. To handle the common rate, the first step is to deliver $\min \{ R_{01}, R_{02} \}$ using the transmission strategy of the multicast problem of  Fig.~\ref{Fig:ExSymmetric}(a). The next steps will follows from using IC and IC with swapped IDs to deliver private messages. Finally, the remaining common rate at one of the transmitters, will be delivered through the strategy of BCs with common rate, and simultaneously, the other transmitter communicates its messages. 
 
In summary, in this section, we presented the transmission strategy for $\mathcal{C}_{\sf SUM}\left( R_0 \right)$ where $0 \leq R_0 \leq (1-q^2)$. We also discussed and highlighted the strategy for other corner points of the capacity region. This completes the proof of Theorem~\ref{THM:Out_XC}.}


==> Camera Ready/Converse_RLBC.tex <==
\noindent {\bf Overview}: The proof is based on the following three key ingredients: (1) for $\msf{Rx}_F$, we find a set of channels realizations that result in the same feedback sequence as the original channel; (2) within this set, we find a candidate that has the same marginal distribution as $S_F^n$ but is maximally correlated with $S_N^n$; (3) as further discussed later, we use the fact that: 
\begin{align}
H(X^n|S_F^n, K^n) = H(X^n|K^n).
\end{align}

\noindent {\bf Derivation}: To derive the outer-bounds, we enhance the knowledge at $\msf{Rx}_N$ by providing it with $S_F^{t-1}$ rather than $K^{t-1}$. The transmitter is still informed causally of the CSI associated with $\msf{Rx}_F$ through a rate-limited feedback link of capacity $C_{\sf FB}$. The proof is broken into several steps as discussed below.

\noindent {\bf Step~1}: From Rate-Distortion Theory, we know that for a binary source distributed as i.i.d. $\mathcal{B}\lp 1-\dl \rp$, given a channel capacity of $C_{\sf FB}$, the minimum attainable Hamming distortion, $0 \leq D^\ast \leq \min\lbp \dl, 1-\dl \rbp$, between the source $S_F^n$ and the estimate $\hat{S}_F^n$, is the solution to~\eqref{Eq:MinDistortion}.
%\begin{align}
%H(D) = \lp H\lp \delta \rp -  C_{\sf FB} \rp^+.
%\end{align}  
%Denote this unique solution by $D^\ast$.

%\begin{remark}
%We note that this argument is for obtaining the outer-bounds, and the transmitter {\bf does not necessarily have to create such an estimate} depending on the strategy used. 
%\end{remark}

Fix the feedback strategy mapping $S_F^n$ to $K^n$, and suppose this strategy results in distortion, $D_{\sf FB} \geq D^\ast$, between $S_F^n$ and the estimate $\hat{S}_F^n$. We further denote the fraction of time instants in which $S_F[t] = 1$ and $\hat{S}_F[t] = 0$ by $D_{10}$. Similarly,  $D_{01}$ is the fraction of time instants in which $S_F[t] = 0$ and $\hat{S}_F[t] = 1$. Thus, we have
\begin{align}
D_{10} + D_{01} =  D_{\sf FB}.
\end{align}

\begin{claim}
\label{Claim:Conditions}
There exists $\tilde{S}_F^n$ such that: $(1)$ we have
\begin{align}
\label{Eq:TildeConditions}
\tilde{S}_F[t] \overset{i.i.d.}\sim \mathcal{B}\lp 1-\dl \rp \text{~and~} \mathbb{E}\lp d\lp \hat{S}_F^n, \tilde{S}_F^n \rp \rp  \leq D_{\sf FB},
\end{align}
where $d\lp \cdot, \cdot \rp$ is the Hamming distance; $(2)$ the feedback encoder maps $\tilde{S}_F^n$ to the same feedback sequence $K^n$ for $S_F^n$. 
\end{claim}

\begin{proof}
Suppose no such sequence exists. Then, the transmitter could have an estimate of $S_F^n$ with a distortion smaller than $D_{\sf FB}$, which would be in contradiction with Rate-Distortion Theory, thus, proving the result. 
\end{proof}

As noted, $\tilde{S}_F[t] \overset{i.i.d.}\sim \mathcal{B}\lp 1-\dl \rp$. Denote the fraction of time instants in which $\tilde{S}_F[t] = 1$ and $\hat{S}_F[t] = 0$  by $\tilde{D}_{10}$, and  the fraction of time instants in which $\tilde{S}_F[t] = 0$ and $\hat{S}_F[t] = 1$ by $\tilde{D}_{01}$. We have
%\begin{align}
$\tilde{D}_{10} + \tilde{D}_{01} \leq D_{\sf FB}$.
%\end{align}
 
\noindent {\bf Step~2}: In this step, we claim if we replace sequence $S_F^n$ with $\tilde{S}_F^n$, the capacity region remains unchanged.

\begin{claim}
\label{Claim:ModifiedBC_RLBC}
Any achievable $\lp R_F, R_N \rp$ is included in the capacity region of a BEC with $\tilde{S}_F^n$ instead of $S_F^n$ while other parameters are kept the same and vice versa.
\end{claim}

\noindent \emph{Proof.} $I\lp W_F; Y_F^n | S_F^n \rp  = I\lp W_F; Y_F^n | S_F^n, K^n \rp$
\begin{align}
%I&\lp W_F; Y_F^n | S_F^n \rp  = I\lp W_F; Y_F^n | S_F^n, K^n \rp  \\
= I\lp W_F; \tilde{Y}_F^n | \tilde{S}_F^n, K^n \rp = I\lp W_F; \tilde{Y}_F^n | \tilde{S}_F^n \rp,
\end{align}
and $I\lp W_N; Y_N^n | S_F^n, S_N^n \rp = I\lp W_N; Y_N^n | S_F^n, S_N^n , K^n \rp$
\begin{align}
%& I\lp W_N; Y_N^n | S_F^n, S_N^n \rp = I\lp W_N; Y_N^n | S_F^n, S_N^n , K^n \rp  \\
& = I\lp W_N; Y_N^n | S_N^n , K^n \rp = I\lp W_N; Y_N^n | \tilde{S}_F^n, S_N^n , K^n \rp.
\end{align}
%\hfill  \hbox

\begin{comment}

\begin{proof}
\begin{align}
I&\lp W_F; Y_F^n | S_F^n \rp  = I\lp W_F; Y_F^n | S_F^n, K^n \rp  \\
&= I\lp W_F; \tilde{Y}_F^n | \tilde{S}_F^n, K^n \rp = I\lp W_F; \tilde{Y}_F^n | \tilde{S}_F^n \rp, \nonumber
\end{align}
and
\begin{align}
& I\lp W_N; Y_N^n | S_F^n, S_N^n \rp = I\lp W_N; Y_N^n | S_F^n, S_N^n , K^n \rp  \\
& = I\lp W_N; Y_N^n | S_N^n , K^n \rp = I\lp W_N; Y_N^n | \tilde{S}_F^n, S_N^n , K^n \rp.\nonumber
\end{align}
\end{proof}

\end{comment}

\noindent {\bf Step~3}: In the rate-limited broadcast channel of Section~\ref{Section:Problem_RLBC}, $S_F[t]$ and $S_N[t]$ are distributed as independent Bernoulli random variables, and the feedback encoder at $\msf{Rx}_F$ is unaware of $S_N^n$. In this step, we create a ``worst-case'' scenario by creating maximum correlation between $S_N^n$ and $\tilde{S}_F^n$.

\begin{claim}
Under the conditions expressed in Claim~\ref{Claim:Conditions}, we have
\begin{align}
\label{Eq:MaxOff}
&\max_{\tilde{D}_{10} + \tilde{D}_{01} \leq D_{\sf FB}} \Pr \lp \tilde{S}_F[t] = S_N[t] = 0 \rp \nonumber \\
&~=\left\{ \begin{array}{ll}
\vspace{1mm} \dl^2 + D_{\sf FB}\lp 1 - \dl \rp, & \min \lbp \dl, 1-\dl \rbp = \dl, \\ %D_{10}
\dl^2 + D_{\sf FB}\dl, & \min \lbp \dl, 1-\dl \rbp = 1 - \dl. %D_{01}
\end{array} \right.
\end{align}
\end{claim}

\begin{figure}[!ht]
\centering
\includegraphics[width = \columnwidth]{FiguresPDF/States.pdf}
\caption{Four possible channel realizations at each time.\label{Fig:Transition}}
%\vspace{-6mm}
\end{figure}

\begin{proof} We divide the proof into two parts based on $\dl$.

\noindent $\bullet$ ${\min \lbp \dl, 1-\dl \rbp = \dl:}$ In this case, to maximize $\Pr \lp \tilde{S}_F[t] = S_N[t] = 0 \rp$, the transition from $S_F^n$ to $\hat{S}_F^n$ would be such that to minimize the times in which $\hat{S}_F[t] = 1$ and $S_N[t] = 0$ by setting $D_{10}\lp 1 - \dl \rp n$ ones to zeros when $S_F[t] = 1$ and $S_N[t] = 0$. The transition from $\hat{S}_F^n$ to $\tilde{S}_F^n$ would be such that to maximize the times in which $\tilde{S}_F[t] = 1$ and $S_N[t] = 1$ by changing $D_{10}\lp 1 - \dl \rp n$ zeros in $\hat{S}_F^n$ to ones when $S_F[t] = 0$ and $S_N[t] = 1$. In effect, such transition from $S_F^n$ to $\tilde{S}_F^n$, increases the probability of $\tilde{S}_F[t] = S_N[t] = 0$ by $D_{10}\lp 1 - \dl \rp$, and since $D_{10} \leq D_{\sf FB}$, the maximum occurs at  $D_{10} = D_{\sf FB}$. Based on Figure~\ref{Fig:Transition}, the discussion above can be explained as follows. The transition from $S_F^n$ to $\hat{S}_F^n$ removes realizations from state $(b)$ and adds them to state $(d)$, while transition from $\hat{S}_F^n$ to $\tilde{S}_F^n$ moves realizations from state $d$ to $(c)$. Thus, end-to-end transitions are from state $(b)$ to $(c)$.  % transition b ---> c

\noindent $\bullet$ ${\min \lbp \dl, 1-\dl \rbp = 1 - \dl:}$ In this case, to maximize $\Pr \lp \tilde{S}_F[t] = S_N[t] = 0 \rp$, the transition from $S_F^n$ to $\hat{S}_F^n$ would be such that to maximize the times in which $S_F[t] = 1$ and $S_N[t] = 1$ by changing $D_{01} \dl n$ zeros to ones when $S_F[t] = 0$ and $S_N[t] = 1$. The transition from $\hat{S}_F^n$ to $\tilde{S}_F^n$ would be such that to minimize the times in which $\tilde{S}_F[t] = 1$ and $S_N[t] = 0$ by changing $D_{01}\dl n$ ones in $\hat{S}_F^n$ to zeros when $S_F[t] = 1$ and $S_N[t] = 0$. In effect, such transition from $S_F^n$ to $\tilde{S}_F^n$, increase the probability of $\tilde{S}_F[t] = S_N[t] = 0$ by $D_{01}\dl$, and since $D_{01} \leq D_{\sf FB}$, the maximum occurs at  $D_{01} = D_{\sf FB}$.
\end{proof}

To prepare for the final step, we define
\begin{align}
\tilde{\gamma}_{\mrm{out}} \overset{\triangle}= \frac{D_{\sf FB}}{\min \lbp \dl, 1-\dl \rbp}.
\end{align}
Based on this definition and \eqref{Eq:MaxOff}, we have
\begin{align}
&\min_{\tilde{D}_{10} + \tilde{D}_{01} \leq D_{\sf FB}} \Pr\left( \{ \tilde{S}_F[t] =  S_N[t] = 0 \}^{c} \right) \nonumber \\
&~= \tilde{\gamma}_{\mrm{out}} \lp 1 - \dl \rp + \lp 1 - \tilde{\gamma}_{\mrm{out}} \rp \lp 1 - \dl^2 \rp.
\end{align}
Further, from rate-distortion theory, we have $D_{\sf FB} \geq D^\ast$. Thus, for {\it any} feedback strategy, we have
\begin{align}
\label{Eq:MaxMin}
&A \overset{\triangle}=\max_{D_{\sf FB} \geq D^\ast} \min_{\tilde{D}_{10} + \tilde{D}_{01} \leq D_{\sf FB}} \Pr\left( \{ \tilde{S}_F[t] =  S_N[t] = 0 \}^{c} \right) \nonumber \\
&~= \gamma_{\mrm{out}} \lp 1 - \dl \rp + \lp 1 - \gamma_{\mrm{out}} \rp \lp 1 - \dl^2 \rp, 
\end{align}
where $\gamma_{\mrm{out}}$ is defined in \eqref{Def:Gamma}, and this bound is attained for a code that achieves the rate-distortion bound. In other words, for {\it any} feedback strategy, we have
\begin{align}
&\Pr\left( \{ \tilde{S}_F[t] =  S_N[t] = 0 \}^{c} \right) \nonumber \\
&~\leq \gamma_{\mrm{out}} \lp 1 - \dl \rp + \lp 1 - \gamma_{\mrm{out}} \rp \lp 1 - \dl^2 \rp
\end{align}
where $\tilde{S}_F^n$ satisfies the conditions in \eqref{Eq:TildeConditions}.




\noindent {\bf Step~4}: For the final step, we first prove the following result.

\begin{claim}
\label{Claim_beta_RLBC}
For the two-user BEC with rate-limited feedback as  described in Section~\ref{Section:Problem_RLBC} and for any input distribution, we have
% adhering to the encoding constraints
\begin{align}
H\left( Y_F^n|W_N,S_F^n,S_N^n \right) - \beta_{\mrm{out}} H\left( Y_N^n|W_N,S_F^n,S_N^n \right) \leq 0,
\end{align}
where $\beta_{\mrm{out}}$ is given in \eqref{Eq:Beta_RLBC}.
\end{claim}

% Suppose $\min \lbp \dl, 1-\dl \rbp = 1-\dl$. Then, the $\lp 1-\dl \rp \tilde{D}$ bits that differ between $\tilde{S}_1^n$ and $S_1^n$ such that $S_1[t] = 1$ and $\tilde{S}_1[t] = 0$, increase the overlap between $\tilde{S}_1^n$ and $S_2^n$ by creating $\tilde{S}_1[t] = 1$, when $S_1[t] = 0$ and $S_2[t] = 1$. In other words, $\tilde{S}_1^n$ and $S_2^n$ become fully correlated fraction $\tilde{\gamma}_{\mrm{out}}$ of times and remain independent a fraction $\lp 1 - \tilde{\gamma}_{\mrm{out}} \rp$ of times.

\begin{proof}
\begin{align}
&H\left( Y_N^n|W_N,S_F^n,S_N^n \right) \nonumber \\
& = H\left( Y_N^n|W_N,S_F^n,K^n,S_N^n \right) \overset{(a)}= H\left( Y_N^n|W_N,K^n,S_N^n \right) \nonumber \\
& = H\left( Y_N^n|W_N,\tilde{S}_F^n,K^n,S_N^n \right) + I\left( Y_N^n; \tilde{S}_F^n|W_N,K^n,S_N^n \right) \nonumber \\
& \overset{(b)}= H\left( Y_N^n|W_N,\tilde{S}_F^n,K^n,S_N^n \right) \overset{(c)}= H\left( Y_N^n|W_N,\tilde{S}_F^n,S_N^n \right) \nonumber \\
& \overset{(d)}= \sum_{t=1}^{n}{H\left( Y_N[t]|Y_N^{t-1},W_N,\tilde{S}_F^t,S_N^t \right)} \nonumber \\
& \overset{(e)}= \sum_{t=1}^{n}{(1-\dl)H\left( X[t]|Y_N^{t-1},W_N,\tilde{S}_F^t, S_N[t]=1,S_N^{t-1} \right)} \nonumber \\
& \overset{(f)}= \sum_{t=1}^{n}{(1-\delta)H\left( X[t]|Y_N^{t-1},W_N,\tilde{S}_F^{t},S_N^t \right)} \nonumber \\
& \overset{(g)}\ge \sum_{t=1}^{n}{(1-\delta)H\left( X[t]|\tilde{Y}_F^{t-1},Y_N^{t-1},W_N,\tilde{S}_F^{t},S_N^t \right)} \nonumber \\
& \overset{(h)} \ge \sum_{t=1}^{n}\frac{(1-\delta)}{A}H\left( \tilde{Y}_F[t], Y_N[t] |\tilde{Y}_F^{t-1},Y_N^{t-1},W_N,\tilde{S}_F^{t},S_N^t \right) \nonumber 
\end{align}
\begin{align}
& \overset{\eqref{Eq:MaxMin}} \ge \sum_{t=1}^{n}{\frac{(1-\delta)H\left( \tilde{Y}_F[t], Y_N[t] |\tilde{Y}_F^{t-1},Y_N^{t-1},W_N,\tilde{S}_F^{t},S_N^t \right)}{\gamma_{\mrm{out}} \lp 1 - \dl \rp + \lp 1 - \gamma_{\mrm{out}} \rp \lp 1 - \dl^2 \rp}} \nonumber \\
& \overset{(\ref{Eq:Beta_RLBC})}= \sum_{t=1}^{n}{\frac{1}{\beta_{\mrm{out}}}H\left( \tilde{Y}_F[t], Y_N[t] |\tilde{Y}_F^{t-1},Y_N^{t-1},W_N,\tilde{S}_F^{t},S_N^t \right)} \nonumber \\
& \overset{(i)}= \sum_{t=1}^{n}{\frac{1}{\beta_{\mrm{out}}}H\left( \tilde{Y}_F[t], Y_N[t] |\tilde{Y}_F^{t-1},Y_N^{t-1},W_N,\tilde{S}_F^{n},S_N^n \right)} \nonumber \\
&= \frac{H\left( \tilde{Y}_F^n, \tilde{Y}_N^n |W_N,\tilde{S}_F^{n},S_N^n \right)}{\beta_{\mrm{out}}} \overset{(j)}\ge \frac{H\left( \tilde{Y}_F^n|W_N,\tilde{S}_F^{n},S_N^n \right)}{\beta_{\mrm{out}}} \nonumber \\
&\overset{\mathrm{Claim}~\ref{Claim:ModifiedBC_RLBC}}\ge \frac{1}{\beta_{\mrm{out}}}H\left( Y_F^n|W_N,S_F^{n},S_N^n \right), 
\end{align}
where $(a)~\&~(b)$ hold since conditioned on $K^{t-1}$, $X[t]$ is independent of all other channel parameters; $(c)$ follows the fact that $\tilde{S}_F^n$ results in $K^n$; $(d)$ follows from the chain rule and the causality of the channel; $(e)$ holds since $S_N[t]$ is a Bernoulli $\left( 1 - \delta \right)$ process; $(f)$ is true since $X[t]$ is independent of channel realizations at time instant $t$; $(g)$ holds since conditioning reduces entropy; $(h)$ follows by the definition of $A$ in \eqref{Eq:MaxMin}, normalizing by the probability that at least one signal is not erased, and ensuring the inequality holds for any feedback strategy; $(i)$ follows the causality assumption; and $(j)$ holds as the discrete entropy function is non-negative.
\end{proof}

Finally, we are ready to prove the outer-bounds.
\begin{align}
&n \left( R_F + \beta_{\mrm{out}} R_N \right) = H\left(W_F\right) + \beta_{\mrm{out}} H\left(W_N\right) \\
& = H\left( W_F|W_N,S_F^n,S_N^n \right) + \beta_{\mrm{out}} H\left( W_N|S_F^n,S_N^n \right) \nonumber \\
& \overset{\mathrm{Fano}}\leq I\left( W_F; Y_F^n|W_N,S_F^n,S_N^n \right) \nonumber \\
&+ \beta_{\mrm{out}} I\left( W_N; Y_N^n|S_F^n,S_N^n \right) + n \epsilon_n \nonumber \\
& = H\left( Y_F^n|W_N,S_F^n,S_N^n \right) - \underbrace{H\left( Y_F^n|W_F,W_N,S_F^n,S_N^n \right)}_{=~0} \nonumber \\
&+ \beta_{\mrm{out}} H\left( Y_N^n|S_F^n,S_N^n \right) - \beta_{\mrm{out}} H\left( Y_N^n|W_N,S_F^n,S_N^n \right) + n \epsilon_n \nonumber \\
& \overset{\mathrm{Claim}~\ref{Claim_beta_RLBC}}\leq \beta_{\mrm{out}} H\left( Y_N^n|S_F^n,S_N^n \right) + n \epsilon_n \leq n \beta_{\mrm{out}} (1-\delta) + n \epsilon_n, \nonumber 
% \nonumber \\
% & \overset{(b)}\leq n \beta_2 (1-\delta_2) + n \epsilon_n,
\end{align}
where $\epsilon_n \rightarrow 0$ as $n \rightarrow \infty$. Dividing both sides by $n$ and taking the limit for $n \rightarrow \infty$ completes the proof. The other outer-bound in Theorem~\ref{THM:Out_RLBC} can be obtained similarly.


















\begin{comment}
%%%%%%%%
Suppose the best estimate of $S_1^n$ that can be reconstructed from $K^n$ is $\hat{S}_1^n$. Then, we have
\begin{align}
\min \mathbb{E}\lp d\lp S_1^n, \hat{S}_1^n \rp \rp  \geq D,
\end{align}
where $d\lp \cdot, \cdot \rp$ is the Hamming distance.

\noindent {\bf Step~2}: Improve to $D$.

Let $D_{0 \rightarrow 1}$ denote the number of time instances in which $S_1[t] = 0$ but $\hat{S}_1[t] = 1$, and similarly, $D_{1 \rightarrow 0}$ denote the number of time instances in which $S_1[t] = 1$ but $\hat{S}_1[t] = 0$. Since the total distortion is $D$, we have 
\begin{align}
D_{0 \rightarrow 1}+D_{1 \rightarrow 0} = D.
\end{align}

\noindent {\bf Step~3}: Suppose $\tilde{S}_1[t]$ is another i.i.d. $\mathcal{B}\lp 1-\dl \rp$ process such that the distortion between $S_1^n$ and $\tilde{S}_1^n$ is $\tilde{D} = D$, and
\begin{align}
%\label{Eq:TildeConditions}
&\tilde{D}_{0 \rightarrow 1} = D_{0 \rightarrow 1} \nonumber \\
&\tilde{D}_{1 \rightarrow 0} = D_{1 \rightarrow 0}.
\end{align} 

\begin{claim}
There exists $\tilde{S}_1^n \neq S_1^n$ satisfying the conditions described above such that the feedback symbols remain unchanged.
\end{claim}

\noindent {\bf Step~4}: New channel

\begin{claim}
Any achievable $\lp R_1, R_2 \rp$ is included in the capacity region of a BC with $\tilde{S}_1^n$ instead of $S_1^n$ while other parameters are kept the same.
\end{claim}  


\noindent {\bf Step~5}:

\begin{claim}
There exists $\tilde{S}_1^n$ satisfying \eqref{Eq:TildeConditions} such that
\begin{align}
\Pr\left( \{ \tilde{S}_1[t] =  S_2[t] = 0 \}^{c} \right) = \gamma_{\mrm{out}} \lp 1 - \dl \rp + \lp 1 - \gamma_{\mrm{out}} \rp \lp 1 - \dl^2 \rp, \nonumber.
\end{align}
\end{claim}
%%%%%%%
\end{comment}


==> Camera Ready/Introduction_RLBC.tex <==
Feedback bandwidth and uplink signaling pose a significant challenge in the development of the next generation of wireless protocols. Many approaches rely on channel state information at the senders to provide better spectral efficiency which quickly becomes a daunting task in large-scale and dynamic systems. For instance, learning channel matrices in  massive MIMO  systems in itself is a challenging task and providing this information to other nodes requires significant reliable feedback bandwidth. However, feedback links are inherently low-rate, local, and unreliable. To make matters more complicated, there is a growing concern about security attacks on feedback and control channels. Thus, it is of great importance to understand the fundamental limits of communications with very low rate local feedback.

%For instance, in 5G where massive MIMO is among the most compelling solution as conventional technology has proven unable to deliver the spectral efficiencies that 5G applications demand. But there remain challenges in adopting massive MIMO in everyday use. The ultimate limit is dictated by mobility since every coherence interval needs to accommodate uplink pilots, and payload in the uplink and downlink directions. The higher mobility, the less channel coherence and the fewer pilots can be afforded. Moreover, as the number of antennas grow to provide better spectral efficiency so does the amount of required uplink signaling to learn the channel.  

%There are several results starting with~\cite{vahid2012interference} that consider wireless networks with rate-limited channel output feedback. But in these setting, the channel is typically assumed to be constant. In (fast) fading networks or in networks with high mobility, an appropriate model is to assume that the transmitters learn the channel state information (CSI) with delay. But even this model does not help with the challenge of uplink signaling overhead. In other words, delay in learning does not reduce the bandwidth required to learning large matrices with complex-valued entries. In this work, we study networks with delayed channel state information at the transmitters (delayed CSIT) and seek to find forward communication protocols that rely on bare minimum feedback. 

% Motivated by these challenges, we study and develop opportunistic uplink signaling mechanisms that use minimal feedback bandwidth. Determining the impact of rate-limited feedback on the capacity region and the communications protocols of general large-scale networks is a distant goal. In this work, we study this problem in the context of the canonical two-user erasure broadcast channels. In fact, if such understanding is not established, there is little hope in solving more general cases. Moreover, the two-user erasure broadcast channel has attracted lots of attention in recent years under various assumptions on feedback availability. 


==> Camera Ready/Main_RLBC.tex <==
In this section, we provide the new distortion-based outer-bound for the two-user BEC with rate-limited feedback. Define $0 \leq D^\ast \leq \min\lbp \dl, 1-\dl \rbp$ to be the unique value to satisfy
\begin{align}
\label{Eq:MinDistortion}
H\lp D \rp = \lp H\lp \delta \rp -  C_{\sf FB} \rp^+,
\end{align}
and $\gamma_{\mrm{out}}$ to be
\begin{align}
\label{Def:Gamma}
\gamma_{\mrm{out}} \overset{\triangle}= \frac{D^\ast}{\min \lbp \dl, 1-\dl \rbp}.
%\gamma_{\mrm{in}} \overset{\triangle}= \frac{\lp H\lp \delta \rp -  C_{\sf FB} \rp^+}{H\lp \delta \rp}.
\end{align}

% Based on these definitions, we set
%\begin{align}
%\label{Eq:Beta_RLBC}
%\beta_{\mrm{out}} &= \gamma_{\mrm{out}} + \lp 1 - \gamma_{\mrm{out}} \rp \lp 1 + \dl \rp, 
%\beta_{\mrm{in}} &= \gamma_{\mrm{in}} + \lp 1 - \gamma_{\mrm{in}} \rp \lp 1 + \dl \rp.
%\end{align}


%The following theorem establishes the outer-bound.
\begin{theorem}
\label{THM:Out_RLBC}
The capacity region, $\mathcal{C}$, of the two-user BEC with one-sided rate-limited feedback is included in
\begin{equation}
\label{Eq:Cout-RLBC}
\mathcal{C}_{\mrm{out}} \overset{\triangle}=
\left\{ \begin{array}{ll}
\hspace{-1.5mm} \left( R_F, R_N \right) \left| \parbox[c][3em][c]{0.25\textwidth} {
$R_F + \beta_{\mrm{out}} R_N \leq \beta_{\mrm{out}} \left( 1 - \delta \right)$\\
$\beta_{\mrm{out}} R_F + R_N \leq \beta_{\mrm{out}} \left( 1 - \delta \right)$
} \right. \end{array} \right\},
\end{equation}
where
\begin{align}
\label{Eq:Beta_RLBC}
\beta_{\mrm{out}} &= \gamma_{\mrm{out}} + \lp 1 - \gamma_{\mrm{out}} \rp \lp 1 + \dl \rp. 
\end{align}
\end{theorem}

Similar to the findings of~\cite{lin2019no}, although only $\msf{Rx}_F$ provides feedback, the outer-bounds are symmetric. The results could also provide new capacity bounds for erasure interference channels based on their connection to BECs~\cite{vahid2012binary,AlirezaBFICDelayed,AlirezaInfocom2014,vahid2018arq}.

Figure~\ref{Fig:SumRateRLBC} plots the outer-bound on the maximum sum-rate point for $\delta = 0.4$.
%, \emph{i.e.} the outer-bound on
%\begin{align}
%\max_{R_F=R_N}{R_F+R_N}.
%\end{align}
When $C_{\sf FB} \geq H\lp \dl \rp$, this outer-bound matches the capacity region of the two-user BEC with global delayed feedback~\cite{gatzianas2013multiuser}. This recovers the results of~\cite{lin2019no,JournalsingleuserCSI} where it is shown that perfect one-sided feedback is as good as global feedback. The interesting distinction between the results in~\cite{lin2019no,JournalsingleuserCSI} and prior results is the fact that delayed CSI is harnessed at every step of the achievability. One can envision a Markov block structure to interleave different blocks and compress the feedback to $H\lp \dl \rp n$ bits and mimic the results of~\cite{lin2019no} to achieve of point ${\sf A}$ in Figure~\ref{Fig:SumRateRLBC} where $H\lp \delta \rp =  C_{\sf FB}$. However, below this limit, the achievability can no longer be derived from such arguments. In fact, the argument presented above requires perfect delayed CSI, and for $C_{\sf FB} < H\lp \dl \rp$, if we attempt to send perfectly a part of CSI back to the transmitter, we deviate from this outer-bound as in  Figure~\ref{Fig:SumRateRLBC}. This suggests the possibility of new achievability ideas that purposefully induce distortion in the encoded CSI.

\begin{figure}[!t]
\centering
\includegraphics[width = \columnwidth]{FiguresPDF/Sum-Rate.pdf}
\caption{Sum-rate outer-bound for $\delta = 0.4$. Point $A$ is where $H\lp \delta \rp =  C_{\sf FB}$.\label{Fig:SumRateRLBC}}
\vspace{-3mm}
\end{figure}


\begin{comment}
\begin{theorem}
\label{THM:In_RLBC}
The following rate region is achievable for the two-user erasure BC with one-sided rate-limited feedback
\begin{equation}
\label{Eq:Rin-RLBC}
\mathcal{R}_{\mrm{in}} =
\left\{ \begin{array}{ll}
\hspace{-1.5mm} \left( R_1, R_2 \right) \left| \parbox[c][3em][c]{0.25\textwidth} {
$R_1 + \beta_{\mrm{in}} R_2 \leq \beta_{\mrm{in}} \left( 1 - \delta \right)$\\
$\beta_{\mrm{in}} R_1 + R_2 \leq \beta_{\mrm{in}} \left( 1 - \delta \right)$
} \right. \end{array} \right\}
\end{equation}
\end{theorem}
\end{comment}




==> Camera Ready/Problem_RLBC.tex <==
We consider the two-user broadcast erasure channel (BEC) of Fig.~\ref{Fig:BC_CEE} in which a single-antenna transmitter, $\msf{Tx}$, wishes to communicate two independent messages, $W_F$ and $W_N$, to two single-antenna receiving terminals $\msf{Rx}_F$ and $\msf{Rx}_N$ (read feedback/silent receiver), respectively, over $n$ channel uses. Each of the messages, $W_F$ and $W_N$, is uniformly distributed over $\lbp1,2,\ldots,2^{nR_F}\rbp$ and $\lbp1,2,\ldots,2^{nR_N}\rbp$, respectively. At time instant $t$, the messages are mapped to channel input $X[t] \in \mathbb{F}_2$ (in the binary field), and the respective received signals at $\msf{Rx}_F$ and $\msf{Rx}_N$ are:
\begin{align}
\label{eq_DL_channel}
Y_F[t] = S_F[t] X[t]~~ \; \mbox{and} \;~~ Y_N[t] = S_N[t] X[t], 
\end{align}
where $\lbp S_F[t]\rbp$ is the Bernoulli $(1-\delta_F)$ process that governs the erasure at $\mathsf{Rx}_F$, and $\lbp S_N[t]\rbp$ is the Bernoulli $(1-\delta_N)$ process that governs the erasure at $\mathsf{Rx}_N$. In this manuscript, we assume the channels are distributed independently over time and across users, and we limit the scope to $\delta_F = \delta_N = \delta$ (\emph{i.e.} homogeneous channels) where $\delta$ is known globally. 

We assume that at time instant $t$, each receiver knows its channel value instantly, \emph{e.g.}, at time instant $t$, $\msf{Rx}_F$ knows the realization of $S_F[t]$. When the channel realization is $1$, the corresponding terminal receives $X[t]$ noiselessly, and when it is $0$, the terminal understands an erasure has occurred. % Note that this is an alternative view of erasure compared to the classical $\{ 0, e, 1 \}$ notation and results in an equivalent representation of erasure channels. 

\begin{figure}[!ht]
\centering
\includegraphics[height = .5\columnwidth]{FiguresPDF/BC-RateLimited.pdf}
\caption{Two-user BEC with rate-limited one-sided feedback.\label{Fig:BC_CEE}}
\end{figure}


\begin{comment} 
We assume forward channels are distributed independently over time, but may have a general distribution across users. In particular, we assume 
\begin{align}
\label{Eq:DeltaFF}
\delta_{12} \overset{\triangle}= P\{S_1[t]=0,S_2[t]=0\}. 
\end{align}
From basic probability, we have
\begin{align}
\label{Eq:d12condition}
\max \{ \delta_1 + \delta_2 -1, 0 \} \leq \delta_{12} \leq \min \{ \delta_1, \delta_2 \}.
\end{align}
\end{comment}

We further assume a one-sided feedback structure in which at time instant $t$, $\mathsf{Rx}_N$ knows $S_N[t]$ but does \emph{not} share this information with the other nodes. On the other hand, we assume $\mathsf{Rx}_F$ shares its channel state with receiver $\mathsf{Rx}_N$ and the transmitter through a rate-limited feedback channel of capacity $C_{\sf FB}$.
%perfectly, and sends this information through a rate-limited feedback channel of capacity $R_{\sf FB}$ to the transmitter. 
We assume the feedback encoder at $\mathsf{Rx}_F$ sends back feedback symbol $K[t] \in \mathcal{K}[t]$ at time $t$ and this information becomes available to the other nodes at time $t+1$. Here, $\mathcal{K}[t]$ is the feedback alphabet at time $t$. The feedback symbol depends causally on $S_F[t]$, and the cardinality of the feedback alphabets satisfies
\begin{align}
\frac{1}{t}\sum_{\ell = 1}^{t}{\log_2\lp \left| \mathcal{K}[\ell] \right| \rp} \leq C_{\sf FB}, \qquad \forall~1 \leq t \leq n.
\end{align}
%For instance, suppose $R_{\sf FB} = 0.5$ bits per channel use, then one possibility is $\mathcal{K}[t] = \emptyset$ for odd values of $t$ and $\mathcal{K}[t] = \lbp 0, 1\rbp$ for even values of $t$.

The constraint imposed at the encoding function $f_t(.) $ at time index $t$ is
\begin{align} 
\label{eq_enc_function}
X[t] = f_t\lp W_F, W_N, K^{t-1} \rp.
\end{align}

Receivers $\msf{Rx}_F$ and $\msf{Rx}_N$ use decoding functions $\varphi_{F,n}\left( Y_F^n, S_F^n \right)$ and $\varphi_{N,n}\left( Y_2^n, K^n, S_N^n \right)$ to get estimates $\widehat{W}_F$ of $W_F$ and $\widehat{W}_N$ of $W_N$, respectively. An error occurs whenever the estimate does not match the corresponding message. The average probabilities of error are given by 
\begin{align}
\lambda_{F,n} = \mathbb{E}[P(\widehat{W}_F \neq W_F)],~\lambda_{N,n} = \mathbb{E}[P(\widehat{W}_N \neq W_N)], 
\end{align}
where the expectations are taken with respect to the random choice of the transmitted messages.

We say that a rate pair $(R_F,R_N)$ is achievable if there exists a block encoder at the transmitter, and a block decoder at each receiver, such that the average probabilities of error go to zero as the block length $n$ goes to infinity. The capacity region, $\mathcal{C}$, is the closure of the set of achievable rate pairs. 

%\begin{remark}[Available CSIR at Receiver 2]
%In this work, we assume  $\mathsf{Rx}_2$ at time instant $t$ knows both $S_1[t]$ and $S_2[t]$. We could instead assume that this receiver knows $K[t]$ and $S_2[t]$ but this assumption further complicates the proof.
%\end{remark}

==> Introduction_RLBC.tex <==
Feedback bandwidth and uplink signaling pose a significant challenge in the development of the next generation of wireless protocols. Many approaches rely on channel state information at the senders to provide better spectral efficiency which quickly becomes a daunting task in large-scale and dynamic systems. For instance, learning channel matrices in  massive MIMO  systems in itself is a challenging task and providing this information to other nodes requires significant reliable feedback bandwidth. However, feedback links are inherently low-rate, local, and unreliable. To make matters more complicated, there is a growing concern about security attacks on feedback and control channels. Thus, it is of great importance to understand the fundamental limits of communications with very low rate local feedback.

%For instance, in 5G where massive MIMO is among the most compelling solution as conventional technology has proven unable to deliver the spectral efficiencies that 5G applications demand. But there remain challenges in adopting massive MIMO in everyday use. The ultimate limit is dictated by mobility since every coherence interval needs to accommodate uplink pilots, and payload in the uplink and downlink directions. The higher mobility, the less channel coherence and the fewer pilots can be afforded. Moreover, as the number of antennas grow to provide better spectral efficiency so does the amount of required uplink signaling to learn the channel.  

%There are several results starting with~\cite{vahid2012interference} that consider wireless networks with rate-limited channel output feedback. But in these setting, the channel is typically assumed to be constant. In (fast) fading networks or in networks with high mobility, an appropriate model is to assume that the transmitters learn the channel state information (CSI) with delay. But even this model does not help with the challenge of uplink signaling overhead. In other words, delay in learning does not reduce the bandwidth required to learning large matrices with complex-valued entries. In this work, we study networks with delayed channel state information at the transmitters (delayed CSIT) and seek to find forward communication protocols that rely on bare minimum feedback. 

% Motivated by these challenges, we study and develop opportunistic uplink signaling mechanisms that use minimal feedback bandwidth. Determining the impact of rate-limited feedback on the capacity region and the communications protocols of general large-scale networks is a distant goal. In this work, we study this problem in the context of the canonical two-user erasure broadcast channels. In fact, if such understanding is not established, there is little hope in solving more general cases. Moreover, the two-user erasure broadcast channel has attracted lots of attention in recent years under various assumptions on feedback availability. 

